From Fake Perfects to Conversational Imperfects: Exploring Image-Generative AI as a Boundary Object for Participatory Design of Public Spaces

Designing public spaces requires balancing the interests of diverse stakeholders within a constrained physical and institutional space. Designers usually approach these problems through participatory methods but struggle to incorporate diverse perspectives into design outputs. The growing capabilities of image-generative artificial intelligence (IGAI) could support participatory design. Prior work in leveraging IGAI's capabilities in design has focused on augmenting the experience and performance of individual creators. We study how IGAI could facilitate participatory processes when designing public spaces, a complex collaborative task. We conducted workshops and IGAI-mediated interviews in a real-world participatory process to upgrade a park in Los Angeles. We found (1) a shift from focusing on accuracy to fostering richer conversations as the desirable outcome of adopting IGAI in participatory design, (2) that IGAI promoted more space-aware conversations, and (3) that IGAI-mediated conversations are subject to the abilities of the facilitators in managing the interaction between themselves, the AI, and stakeholders. We contribute by discussing practical implications for using IGAI in participatory design, including success metrics, relevant skills, and asymmetries between designers and stakeholders. We finish by proposing a series of open research questions.

==> archive/participant_table.tex <==
\begin{table}[htb]
    \centering
    %First set of interviews.
    \begin{tabular}{p{0.15\linewidth} p{0.2\linewidth} p{0.25\linewidth} p{0.2\linewidth}}
    \toprule
       \multicolumn{4}{c}{\cellcolor{lightgray!20!}\textbf{Interviews from prior work to Immigrants in LA}}\\
       \hline
       Participant & Gender & Country of Origin & Years in LA\\
       \hline
%       \multicolumn{4}{c}{\textbf{Interviews to Immigrants about the design of a Park in Puente Hill Landfill}}\\
%       \hline
       A1 & Male & Mexico & 21-25\\
       A2 & Male & El Salvador & 40+ \\
       A3 & Male & Mexico & 26-30  \\
       A4 & Male & El Salvador & 10-15 \\
       A5 & Male & Mexico & 0-5 \\
       A6 & Female & Mexico & 21-25 \\
       A7 & Female & Chile & 0-5\\
       A8 & Female & Chile & 0-5\\
    \bottomrule
    \end{tabular}
 % Internal Interviews 1st stage
    \begin{tabular}{p{0.15\linewidth} p{0.5\linewidth} p{0.25\linewidth}}
    \toprule
       \multicolumn{3}{c}{\cellcolor{lightgray!20!}\textbf{Stage 1: Internal Interviews}}\\
       \hline
%       \multicolumn{4}{c}{\textbf{User study with potential users}}\\
%       \hline
       Participant & Education & Gender \\
       \hline
       B1 & Ph.D. in Landscape Design Theory and Master in Landscape Architecture & Female\\
       B2 & Master in Architecture \& Master Landscape Architecture & Male \\
       B3 & Master in Landscape Architecture & Female \\
       B4 & Architecture student & Male \\
    \bottomrule
    \end{tabular}
%Workshop 1 Participants
   \begin{tabular}{p{0.15\linewidth} p{0.5\linewidth} p{0.25\linewidth}}
    \toprule
       \multicolumn{3}{c}{\cellcolor{lightgray!20!}\textbf{Stage 1: Reflection Workshop}}\\
       \hline
%       \multicolumn{4}{c}{\textbf{User study with potential users}}\\
%       \hline
       Participant & Education & Gender \\
       \hline
       C1 & Ph.D. in Landscape Design Theory and Master in Landscape Architecture & Female\\
       C2 & Master in Architecture \& Master Landscape Architecture & Male \\
       C3 & Master in Landscape Architecture & Male \\
       C4 & Master in Landscape Architecture Student & Female \\
       C5 & Master in Landscape Architecture Student & Male \\
       C6 & Architecture student & Male \\
       C7 & Ph.D. in Information Science student & Male \\
       C8 & Ph.D. in Engineering and Public Policy & Male \\
       C9 & Ph.D. in Communication & Female \\
    \bottomrule
    \end{tabular}

    %Pilot Interviews
   \begin{tabular}{p{0.15\linewidth} p{0.5\linewidth} p{0.25\linewidth}}
    \toprule
       \multicolumn{3}{c}{\cellcolor{lightgray!20!}\textbf{Stage 2: Piloting Interviews}}\\
       \hline
%       \multicolumn{4}{c}{\textbf{User study with potential users}}\\
%       \hline
       Participant & Education & Gender \\
       \hline
       D1 & Ph.D. in Landscape Design Theory and Master in Landscape Architecture & Female\\
       D2 & Ph.D. in Information Science student & Male \\
       D3 & Ph.D. in Communication & Female \\
    \bottomrule
    \end{tabular}

    %Interviews
       \begin{tabular}{p{0.3\linewidth} p{0.2\linewidth} p{0.3\linewidth}}
    \toprule
       \multicolumn{3}{c}{\cellcolor{lightgray!20!}\textbf{Stage 3: Interviews in LA to 2nd generation immigrants}}\\
       \hline
       Participant & Gender & Immigration origin\\
       \hline
       E1 \& E2 \& E3 \& E4 \& E6 \& E7 & Female & Mexico\\
       E5 & Male & Mexico\\
       E8 & Female & Unknown\\
       E9 & Male & Guatemala\\
       \hline
    \end{tabular}

    %Workshop 2 Participants
   \begin{tabular}{p{0.15\linewidth} p{0.5\linewidth} p{0.25\linewidth}}
    \toprule
       \multicolumn{3}{c}{\cellcolor{lightgray!20!}\textbf{Stage 3: 2nd Reflection Workshop}}\\
       \hline
%       \multicolumn{4}{c}{\textbf{User study with potential users}}\\
%       \hline
       Participant & Education & Gender \\
       \hline
       F1 & Ph.D. in Landscape Design Theory and Master in Landscape Architecture & Female\\
       F2 & Master in Architecture \& Master Landscape Architecture & Male \\
       F3 & Master in Landscape Architecture & Male \\
       F4 & Master in Landscape Architecture Student & Female \\
       F5 \& F6 & Master in Landscape Architecture Student & Male \\
       F7 & Architecture student & Male \\
       F8 & Ph.D. in Information Science student & Male \\
       F9 & Ph.D. in Engineering and Public Policy & Male \\
       F10 & Ph.D. in Communication & Female \\
    \bottomrule
    \end{tabular}
    
    \vspace{0.2cm}
%    \caption{Study Participants (*Values in \textbf{Prof. Exp.} represent participants' professional experience in years)}
    \label{tab:participant}
\end{table}

